VoxDepth: Rectification of Depth Images on Edge Devices

Autonomous mobile robots like self-flying drones and industrial robots heavily depend on depth images to perform tasks such as 3D reconstruction and visual SLAM. However, the presence of inaccuracies in these depth images can greatly hinder the effectiveness of these applications, resulting in sub-optimal results. Depth images produced by commercially available cameras frequently exhibit noise, which manifests as flickering pixels and erroneous patches. ML-based methods to rectify these images are unsuitable for edge devices that have very limited computational resources. Non-ML methods are much faster but have limited accuracy, especially for correcting errors that are a result of occlusion and camera movement. We propose a scheme called VoxDepth that is fast, accurate, and runs very well on edge devices. It relies on a host of novel techniques: 3D point cloud construction and fusion, and using it to create a template that can fix erroneous depth images. VoxDepth shows superior results on both synthetic and real-world datasets. We demonstrate a 31% improvement in quality as compared to state-of-the-art methods on real-world depth datasets, while maintaining a competitive framerate of 27 FPS (frames per second).

==> 2dmethods.tex <==
\subsection{2D Depth Image Correction}
\textcolor{blue}{In a mobile robot, the view seen by the camera is continually changing, hence it is necessary to adjust for this camera motion.}
\subsubsection{Image Registration}
\label{subsubsec:imgreg}
%FIXME: Some continuity is required. Where is this paragraph coming from
Image {\em registration} refers to the process of \underline{aligning}
two distinct images or frames of a shared scene to a common
coordinate system.  In order to accomplish this, we calculate 
the transformation between two frames by comparing the
pixels in the two frames. \textcolor{blue}{In image processing, a transformation refers to the process of applying mathematical operations to an image to change its characteristics or extract specific information, such as altering its geometry, adjusting its intensity values, or converting it to a different domain.}

%FIXME: Break in continuity here 
One such transformation is an affine transformation.
An affine transformation refers to a
geometric transformation that preserves points, straight
lines and planes.  It includes operations such as translation 
(shifting), rotation, scaling (resizing) and shearing
(stretching). It is a common transformation used in image 
registration. An affine transformation can be represented as a
rotation $A$ followed by a translation $b$.  The transformed 
coordinates of the image are as follows:

\begin{equation}
    % \footnotesize
    \label{eqn:trans}
        P_1= A\times P_0 + b
\end{equation}

$P_0$ represents the original coordinates of the pixel, 
and $P_1$ represents the computed (transformed) coordinates. 
In our implementation, 
we condense this transformation using a single $2\times3$ matrix $M$.

%FIXME: Lost focus here

\textcolor{blue}{To estimate an affine transformation, the squared difference between the real image and 
the transformed image is minimized.} 
Formally, if an image is represented as $I(u,v)$, denoting the pixel intensity at the pixel coordinates $(u,v)$,
then we minimize the following objective function: 

\begin{equation}
    % \footnotesize
    \label{eqn:objfun}
    E = \sum_{u,v} \left\|I_1\left(M \begin{bmatrix} u \\ v \\ 1 \end{bmatrix}\right) - I_0\left(\begin{bmatrix} u \\ v \end{bmatrix}\right)\right\|^2
\end{equation}
%FIXME: What is the point of transformation?
\textcolor{blue}{Image registration aides in estimating the motion of the camera and transforming frames compensates for that motion.}
% In order to expedite the registration process, it is suggested to reduce the dimensions of the frames to improve the time it takes to
% find matches.

%FIXME: "We reduce the" is a verb. It cannot appear in the background section. Only basic concepts.

==> 3dmethods.tex <==
\subsection{3D Point Cloud Fusion}
\subsubsection{Point Cloud}
\label{subsubsec:pcd}
Point clouds are three-dimensional data structures composed of points representing the surface of objects or scenes in
the real world.
Let us mathematically represent the RGB-D frames generated by a stereoscopic depth camera.
$I_{RGB}$ represents
the channel-wise RGB intensity and $I_{D}$ is the 
depth of the point in meters 
in the image plane $\gamma \subseteq \mathbb{R}_{+}^{2}$ at point $x\in \gamma$, at time $t \in \mathbb{R}_{+}$.

\begin{equation}
    % \footnotesize
    \label{eqn:rgbframe}
    I_{RGB}:\gamma \times \mathbb{R}_{+} \rightarrow [0,1]^{3}, (x,t) \rightarrow I_{RGB}(x,t)
\end{equation}
\begin{equation}
    % \footnotesize
    \label{eqn:dframe}
    I_{D}:\gamma \times \mathbb{R}_{+} \rightarrow \mathbb{R}_{+}, (x,t) \rightarrow I_{D}(x,t)
\end{equation}

From the depth image $I_D$, we can compute the surface $S$ visible from the sensor by projecting the
points in a 3D space for each point $p=(p_x,p_y)\in\gamma$, $\gamma \subseteq \mathbb{R}_{+}^{2}$ in the depth image at
some point at time $t_0$ (see Equation~\ref{eqn:surface2}). In Equation~\ref{eqn:surface2}, $(o_u,o_v)^{T}$ is the
principal point of the camera on the $x$ and $y$ axis, respectively.

\begin{equation}
    \footnotesize
    \label{eqn:dframe}
    I_{D}:\gamma \times \mathbb{R}_{+} \rightarrow \mathbb{R}_{+}, (p,t) \rightarrow I_{D}(p,t)
\end{equation} 
\begin{equation}
    \footnotesize
    \label{eqn:surface1}
    S:\gamma \rightarrow R^{3},
\end{equation}
\begin{equation}
    \footnotesize
    \label{eqn:surface2}
    S(p)=\left( \dfrac{(p_x+o_u)I_D(p,t_0)}{f_x},\dfrac{(p_y+o_v)I_D(p,t_0)}{f_y},I_D(p,t_0)\right)^{T}
\end{equation}

The {\em principal point} refers to the point on the image plane where the line passing through the center of the camera
lens (optical axis) intersects the image plane. 
The focal lengths in the $x$ and $y$ directions are represented by $f_x$
and $f_y$, respectively.  Each point in the {\em point cloud}
corresponds to a specific position in space and is specified by
its $x$, $y$ and $z$ coordinates. 
To combine multiple such point cloud data structures, we need to transform them to a {\em common coordinate system}.

\subsubsection{RGB-D Odometry}
\label{subsubsec:RGBDodo}
The objective of RGB-D 
odometry is to estimate the rigid body motion $q \in SE(3)$ of the camera given two consecutive images $I(t_0)$ and $I(t_1)$.
This {\em motion} is a transformation with six degrees of freedom: three describe camera rotation (roll, pitch and yaw) and
three represent translation ($x,y,z$).  
Using this transformation, we can align multiple point clouds to a common coordinate system, we
can fuse them together to form a {\em dense point cloud}.

\subsubsection{Point Cloud Fusion}
\label{subsubsec:pcf}
Point cloud {\em fusion} is the process
of aligning and merging point clouds from multiple viewpoints (or sensors) to
build a more complete and accurate 3D model of the scene. RGB-D odometry, described in
Section~\ref{subsubsec:RGBDodo}, is used to align multiple point clouds to a common coordinate system. 
Figures \ref{fig:pointcloud} and \ref{fig:voxelfused} show how multiple point clouds are
merged together to form a more complete and less noisy representation of the scene. In our method, we add an
additional step that involves
{\em reprojecting} the merged point cloud back to a 2D image to create
the (\underline{the template}), by following the reverse sequence of
steps (reverse of
Equation~\ref{eqn:surface2}).

\begin{figure}[!htb]
	\centering
	\subfloat[Point cloud from a single depth image]{
		\includegraphics[width=0.45\columnwidth]{pointcloud.pdf}
		\label{fig:pointcloud}
	}
	\subfloat[Fused point cloud]{
		\includegraphics[width=0.45\columnwidth]{voxelfused.pdf}
		\label{fig:voxelfused}
	}
    % \\
    % \subfloat[Sparse voxel fused depth image]{
    % \includegraphics[width=0.40\columnwidth]{voxel.pdf}
    % }
    % \subfloat[Upsampled depth image]{
    % \includegraphics[width=0.40\columnwidth]{Upsampled.pdf}
    % \label{fig:voxupsample}
    % }
	\caption{Fused point cloud generated after the fusion step. 
    The fusion process fills up holes in the point cloud.}
\end{figure}  

==> cuda.tex <==
\subsection{CUDA Programming Model}
\label{subsec:cuda}
The CUDA programming paradigm~\cite{luebke2008cuda} offers a structured approach for crafting parallel applications designed for execution on NVIDIA GPUs (Graphics Processing Units). By extending the conventional C/C++ programming languages with specialized GPU functionalities, it empowers developers to leverage the immense computational capabilities of GPUs for various general-purpose processing requirements. The key aspects of the CUDA programming model include \circled{1} kernel functions that executed in parallel by multiple threads on GPU, \circled{2} arrangement of threads into grids and blocks which can be tailored  to the specific requirements of the application to maximize GPU utilization and performance, \circled{3} memory models to reduce access latency depending on the task and \circled{4} synchronization to coordinate the operation of parallelly running threads, avoiding race conditions.

\subsection{Unified Memory}
\label{subsec:unified}
Unified Memory, introduced in CUDA, streamlines memory management by offering a unified virtual address space accessible to both the CPU and GPU. This functionality simplifies memory allocation and access, eliminating the need for manual data transfers between CPU and GPU memory spaces. We create a unified memory buffer to store and operate on image data using both CPU and GPU threads. This eliminates the latency associated with copying data from host to device. 

\begin{table*}[!htb]
  \footnotesize
  % \fontsize{20pt}{20pt}\selectfont
  \begin{center}
    \resizebox{1.9\columnwidth}{!}{
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
      \hline
      \multicolumn{2}{c}{\textbf{Method}}& \multicolumn{2}{c}{\textbf{LN}} &  \multicolumn{2}{c}{\textbf{MB}} & \multicolumn{2}{c}{\textbf{KTS}} & \multicolumn{2}{c}{\textbf{KTC}} & \multicolumn{2}{c}{\textbf{PLF}} & \multicolumn{2}{c}{\textbf{PLW}}\\

      \hline
      & Abbr. & PSNR (dB) & M-RMSE & PSNR (dB) & M-RMSE & PSNR (dB) & M-RMSE & PSNR (dB) & M-RMSE & PSNR (dB) & M-RMSE & PSNR (dB) & M-RMSE \\ 
      \hline

    VoxDepth & \textit{VD} & \textbf{17.46} & \textbf{112.25} & \textbf{17.10} & 177.61 & 17.69 & \textbf{102.23} & \textbf{20.32} & \textbf{126.15} & \textbf{15.81} &  \textbf{157.95}  & \textbf{16.05} & 169.79\\
      \hline
    Realsense & \textit{RS~\cite{grunnet2018depth}} & 13.04 & 167.25 & 13.17 & \textbf{175.61} & 14.60 & 139.69 & 17.66 & 144.70 & 13.55 & 159.15 & 13.73 & \textbf{164.79} \\
      \hline
    GSmooth & \textit{GS ~\cite{islam2018gsmooth}}& 13.14 & 179.08 & 15.36 & 176.75 & 19.09 & 172.02 & 18.59 & 177.93 & 12.97 & 178.70 & 13.14 & 177.59 \\
      \hline
    DeepSmooth & \textit{DS~\cite{krishna2023deepsmooth}} & 14.16 & 180.03 & 10.51 & 178.04 & \textbf{22.87} & 175.68 & 14.89 & 178.89 & 13.62 & 178.38 & 13.37 & 178.87   \\
      \hline
    \end{tabular}

    }
    \end{center}
    \caption{Comparison of quality of different methods based on PSNR (dB, higher is better) and M-RMSE (lower is better)}
    \label{tab:psnr}
  \end{table*}

  Our approach involves the efficient utilization of both the GPU and CPU on the board, while also taking into consideration the power consumption. Although a hardware-based solution would be more suitable for larger machines, a software solution is more appropriate for small embedded systems that are already limited by power.\\

  \begin{algorithm}
    \caption{Algorithm to Generate Fused Point Cloud}
    \label{algo:fusion}
    \begin{algorithmic}
      \REQUIRE $\texttt{initWindow}, \texttt{cameraIntrinsic}$
      \ENSURE $\texttt{fusedPC}$
      
      \STATE $\texttt{rgbd1} \leftarrow \text{getRGBDImage}()$
      \STATE $\texttt{rgbd2} \leftarrow \text{copy}(\texttt{rgbd1})$
      \STATE $\texttt{pointCloud} \leftarrow \text{createVoxelPointCloud}(\texttt{rgbd1})$
      \STATE $\texttt{fusedPC} \leftarrow \text{createEmptyVoxelPointCloud}()$
      \STATE $\texttt{transTerm} \leftarrow \text{identityMatrix}(4)$
      
      \FOR{$\texttt{i} \leftarrow  1$ \TO $\texttt{initWindow}$}
        \STATE $\texttt{fusedPC} \leftarrow \text{transform}(\texttt{fusedPC}, \texttt{transTerm})$
        \STATE $\texttt{fusedPC} += \texttt{pointCloud}$
        % \STATE $\texttt{fusedPC} \leftarrow \text{downSample}(\texttt{fusedPC}, 5)$
  
        \STATE $\texttt{rgbd2} \leftarrow \text{getRGBDImage}()$
        \STATE $\texttt{pointCloud} \leftarrow \text{createVoxelPointCloud}(\texttt{rgbd2})$
        \IF{$\texttt{i}=1$}
        \STATE $\texttt{transTerm}\leftarrow \text{computeOdometry}(\texttt{rgbd1}, \texttt{rgbd2})$
        \ENDIF
      \ENDFOR
      
      \STATE $\texttt{fusedPC} \leftarrow \text{transform}(\texttt{fusedPC}, \texttt{transTerm})$
      \STATE $\texttt{fusedPC} += \texttt{pointCloud}$
    \end{algorithmic}
  \end{algorithm}

  % \subsection{Component Latency}
% \label{subsec:latencies}
% In order to establish an effective approach, it is imperative that we strictly adhere to minimizing latency for each of our components. Significant delays can impede the functioning of an autonomous system and lead to unforeseen actions from the robot. 
% In Table~\ref{tab:latencies} we list the latencies of all the major components in our system measured on an Nvidia Jetson Nano developer board. 
% For comparison we also measure the same components on the workstation. We find point cloud fusion to be the biggest contributor of latency in our system. 
% \begin{table}[H]
%   \footnotesize
%   \begin{center}
%     \begin{tabular}{|l|l|l|l|}
%       \hline
%      \textbf{Device} & {\textbf{PC Fusion (ms)}}  & {\textbf{Image Regis. (ms)}} & {\textbf{Depth}} \\
%      & & & {\textbf{correction (ms)}}\\
%      \hline
%       Workstation & 73 & 4 & 3 \\
%       \hline
%       Jetson Nano & 352 & 4 & 15 \\
%       \hline
%     \end{tabular}
%    \end{center}
%    \caption{Latencies of different components. PC - point cloud, DM- depth map}
%     \label{tab:latencies}
%   \end{table}

==> framedegrade.tex <==
\subsection{Frame Degradation Study}
\label{subsec:degrade}
In our method we propose a point cloud fusion module as described in Section~\ref{subsec:pcf}. In this section we run some experiments to see how frequently 
would we need to redo the fusion step to maintain quality. 
We define the frequency of fusion as the reciprocal of the number of frames in between consecutive fusions. 
We plot the quality of the generated frames (measured in peak signal-to-noise ration ~\cite{hore2010image}) against frequency of fusion. We also include 
the PSNR of the corrected frames generated with gSmooth ~\cite{islam2018gsmooth} and the Realsense SDK Hole-filling algorithm ~\cite{grunnet2018depth}. Since there is no 
concept of initialization in the above two methods, their frame quality remains constant. Figure~\ref{degradation}(b) shows the result of our experiment. We see that frequency of fusion is proportional to the quality of the image meaning the more frequently the fusion step is carried out the better is the result.

\subsection{Initialization Window Size}
\label{subsec:initwindo}
The initialization window or init window determines how many frames are considered when creating the fused point cloud. Since fusion is an expensive 
step as shown in Table~\ref{tab:latencies}, we would ideally like to consider as few frames as possible to estimate the scene. We plot the quality of the corrected frame (measured in peak signal-to-noise ration ~\cite{hore2010image}) the number of frames used in the initialization window against the number of frames used in the initialization window in the Figure~\ref{degradation}(b). We see that the larger the init window, the better is the quality of the corrected frame.
\\
\vspace*{-\baselineskip}
\begin{figure}[!htb]
\subfloat[Frame quality vs frequency of fusion]
  {\includegraphics[width=0.90\columnwidth]{sceneInit.pdf}}
  \\
\subfloat[Frame quality vs init window size]
  {\includegraphics[width=0.90\columnwidth]{initwindowsize.pdf}}
\caption{Plots Showing Degradation in corrected frames against varying initialization frequency and Init window size }
\label{degradation}
\vspace{-6mm}
\end{figure}
